Hyperbolic Secant representation of the logistic function: Application to probabilistic Multiple Instance Learning for CT intracranial hemorrhage detection

Multiple Instance Learning (MIL) is a weakly supervised paradigm that has been successfully applied to many different scientific areas and is particularly well suited to medical imaging. Probabilistic MIL methods, and more specifically Gaussian Processes (GPs), have achieved excellent results due to their high expressiveness and uncertainty quantification capabilities. One of the most successful GP-based MIL methods, VGPMIL, resorts to a variational bound to handle the intractability of the logistic function. Here, we formulate VGPMIL using P\'olya-Gamma random variables. This approach yields the same variational posterior approximations as the original VGPMIL, which is a consequence of the two representations that the Hyperbolic Secant distribution admits. This leads us to propose a general GP-based MIL method that takes different forms by simply leveraging distributions other than the Hyperbolic Secant one. Using the Gamma distribution we arrive at a new approach that obtains competitive or superior predictive performance and efficiency. This is validated in a comprehensive experimental study including one synthetic MIL dataset, two well-known MIL benchmarks, and a real-world medical problem. We expect that this work provides useful ideas beyond MIL that can foster further research in the field.

==> sections/discussion.tex <==
\section{Discussion}\label{section:discussion}

Thanks to the work carried out in the theoretical part of this work, we have generalized existing VGPMIL, thus obtaining a general framework with a wide variety of realizations to be explored. The results presented in the experimental section manifest that G-VGPMIL, a realization of such a framework, improves upon the state-of-the-art GP-based MIL methods. Before proceeding to the conclusions, we summarise the main contributions of this work and explore their significance and impact.

%\textcolor{review}{
\textbf{The logistic observation model admits two representations that lead to the same variational updates}. 
The treatment of the logistic observation model is made through the density $\phi$, which belongs to the Generalized Hyperbolic Secant family. 
We have shown that $\phi$ admits two different representations by showing that it is SG and an SMG. 
We have theoretically connected the Jaakkola bound and the Pólya-Gamma variable augmentation approach. 
This connection reveals that both approaches lead to the optimization of the same objective. Thus, they produce the same variational updates when approximating the posterior, which justifies the equivalence between VGPMIL and PG-VGPMIL. 
%}

\textbf{We devise a general inference framework for the logistic observation model.} The equivalence between VGPMIL and PG-VGPMIL leads us to realize that both models are a realization of a general probabilistic framework. The joint probability in this framework is obtained by replacing the logistic observation model in Eq. \eqref{eq:y_prob} with the augmented \eqref{eq:p_y_omega_general}. The particular density associated with the newly introduced variables will determine the realization of the model we obtain. This density does not need to be explicitly defined, but it is sufficient to choose a decreasing function to compute the variational updates. If this density is in the Pólya-Gamma family, we recover the PG-VGPMIL model. On the other hand, if we choose it to be in the Gamma family, we arrive at our G-VGPMIL model. 

\textbf{G-VGPMIL outperforms VGPMIL in terms of performance and training time.} 
%The newly proposed model, G-VGPMIL, shows better prediction performance than the state-of-the-art model VGPMIL in all three problems considered. 
This superiority is achieved in every classification metric considered (Accuracy, F1 and AUC), at both the instance and bag level, and in all three problems considered. Only in the RSNA dataset VGPMIL has presented better results in terms of Accuracy and F1 metrics at the instance level. Also, our experiments show that G-VGPMIL has a faster and more stable convergence. This translates into a reduced training time, and consequently a lower training workload. 

\textbf{G-VGPMIL improves the state-of-the-art results for the ICH detection problem.} The third problem considered consists of the detection of ICH from brain CT scans. As shown in Table \ref{tab:cq500_literature_comparison}, the state-of-the-art results are achieved by fully supervised models that need the label of each slice, which is a daunting annotation effort for radiologists. With this work, we close the gap with them with a model that requires only scan labels and still obtains very competitive results. 

\textbf{Open challenges.} Although G-VGPMIL relies on a strong theoretical formulation and shows many important empirical advantages, it also opens three new challenges to improve the performance of probabilistic MIL methods. The first is related to the role played by Gamma variables, as there are many distributions with important properties that could improve the generalization ability of G-VGPMIL. Furthermore, as the $\theta$ function in Eq. \eqref{eq:theta_mat_val} is the only one involved in the inference process, one may explore the properties that this function must have to increase the capacity of the model. The second challenge is also of theoretical nature. When formulating VGPMIL and G-VGPMIL, we have followed the common assumption of independence across instances in a bag. However, taking into account the order and the relationships among instances should increase the performance of these methods. The last challenge is about the training procedure of G-VGPMIL. As it can not deal with raw images directly, we need to apply a feature extraction procedure before training the model. In this work, we have proposed a two-step approach. However, the features extracted by the attention-based CNN may not be optimal for G-VGPMIL, thus requiring an end-to-end training procedure. Future work will tackle these issues. 
